MSRF-Net: A Multi-Scale Residual Fusion Network for Biomedical Image Segmentation

Methods based on convolutional neural networks have improved the performance of biomedical image segmentation. However, most of these methods cannot efficiently segment objects of variable sizes and train on small and biased datasets, which are common for biomedical use cases. While methods exist that incorporate multi-scale fusion approaches to address the challenges arising with variable sizes, they usually use complex models that are more suitable for general semantic segmentation problems. In this paper, we propose a novel architecture called Multi-Scale Residual Fusion Network (MSRF-Net), which is specially designed for medical image segmentation. The proposed MSRF-Net is able to exchange multi-scale features of varying receptive fields using a Dual-Scale Dense Fusion (DSDF) block. Our DSDF block can exchange information rigorously across two different resolution scales, and our MSRF sub-network uses multiple DSDF blocks in sequence to perform multi-scale fusion. This allows the preservation of resolution, improved information flow and propagation of both high- and low-level features to obtain accurate segmentation maps. The proposed MSRF-Net allows to capture object variabilities and provides improved results on different biomedical datasets. Extensive experiments on MSRF-Net demonstrate that the proposed method outperforms the cutting-edge medical image segmentation methods on four publicly available datasets. We achieve the dice coefficient of 0.9217, 0.9420, and 0.9224, 0.8824 on Kvasir-SEG, CVC-ClinicDB, 2018 Data Science Bowl dataset, and ISIC-2018 skin lesion segmentation challenge dataset respectively. We further conducted generalizability tests and achieved a dice coefficient of 0.7921 and 0.7575 on CVC-ClinicDB and Kvasir-SEG, respectively.

==> takeout.tex <==


 demonstrate that

%not suitable to train on datasets with limited number of samples.
%Our generalization results demonstrate that \sysname can be used as a baseline for biomedical image segmentation. 

%which is especially designed to perform multi-scale fusion in limited medical image segmentation datasets.

%Image segmentation can provide detailed boundary information of macroscopic lesions in medical images and microscopic cellular structures in biological imaging. 



% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi
% \vfill

% \begin{table}[!t]
% \centering
% \scriptsize
% \caption{Ablation study on shape stream}
% \begin{tabular}{l|l|l}
% \toprule
% \textbf{Component} &\textbf{Position} & \textbf{BCE} \\
% \hline
% \hline
% Shape stream &  before MSRF sub-network  & 0.1002 \\ %\hline
% Shape stream &  after MSRF sub-network  & 0.1046 \\ 
% \bottomrule
% \end{tabular}
% \label{tab:abl1}
% \end{table}


%The shape stream's output is computed before the skip-connections are processed by the  \ac{MSRF} sub-network. Then, shape predictions of the shape stream in both the networks. It is to be noted that we have used the same number of parameters in both the models. Finally, we compute and compare quantitative and qualitative results.

%
%The resolution streams $X_{r=1}$,$X_{r=2}$ and $X_{r=3}$,$X_{r=4}$ are able to exchange information amongst themselves. The absence of \ac{DSDF} across $X_{r=2}$ and $X_{r=3}$ prevents global multi-scale fusion~\ref{alg:algo1}. 

%Therefore, we can say that the scaling mechanism in the deployed \ac{DSDF} boosts the segmentation performance. Moreover, scaling was able to prevent instability caused by a large number of parameters in \ac{DSDF}. 

%To achieve global multi-scale context, it is essential that each resolution scale to exchange information with each other. 
%TODO: Put this in supplementary please!
% \begin{figure}[t!]
% \includegraphics[width=0.5\textwidth]{global scale exchange.png}
% \caption{The red line displays how X_{1} is able to exchange its features with all other resolution scales using multiple MSRFRDB's}
% \label{fig:figlobal}
% \end{figure}
%Since incorporating every scale in the DSDF by using $N$ parallel stream's is computationally expensive and to make the training easier we come up with a strategy to exchange multi-scale features globally \ref{alg:algo1}.

%\item DSDF block incorporates exchange of information across different scales allowing both high- and low-resolution information to propagate and compliment the extraction of semantically meaningful features. 





% \subsubsection{Generalizibilty test}
% \begin{table}[t!]
% \centering
% %\scriptsize
% \footnotesize
%  \caption{Generalizability Test}
%     \label{table:generalization}
%     \begin{tabular}{@{}l|l|l|l|l|l@{}}  
%       \toprule
%           \textbf{Train set}&\textbf{Test set} & \textbf{DSC}& \textbf{mIoU} &\textbf{Recall} &\textbf{Precision}\\ \hline
%                 \hline
%                 Kvasir-SEG &CVC-ClinicDB  &0.7921 &0.8079 &0.8465 &0.9365 \\ \hline
%                 CVC-ClinicDB &Kvasir-SEG &0.7575 &0.7825 &0.8481 &0.8970 \\
%                 \bottomrule 
% \end{tabular}

% \end{table}




%From the quantitative results (Table~\ref{tab:generalizationcvc}, \ref{tab:generalizationkvasir}), we can observe that despite using two datasets acquired using two different imaging protocols, our proposed \sysname is able to achieve a \ac{DSC} of 0.7921 and \ac{mIoU} of 0.8079, when trained on Kvasir-SEG and tested on CVC-ClinicDB. Similarly, the \sysname obtained \ac{DSC} of 0.7575 and \ac{mIoU} of 0.7825 when trained on CVCClinincDB and tested on Kvasir-SEG. On the cross-data test set, the results are usually poor. However, the experimental results show that our \sysname achieves competitive generalization results.
%
%\section{Generalization}
%In medical imaging, generalization is the ability of the algorithm trained on specific interventions in specific hospitals that should be able to generalize over other interventions or hospitals~\cite{ross2020robust}. We determine the generalization capability of our proposed \sysname by training on one dataset and testing on another dataset. These experiments are conducted on Kvasir-SEG and CVC-ClinicDB. We compare the generalizibility performance of our proposed \sysname with other \ac{SOTA} methods in (Table~\ref{tab:generalizationcvc}, \ref{tab:generalizationkvasir}). From the quantitative results we are able to show that our proposed \sysname is able to beat other \ac{SOTA} methods in generalizibility performance. 


%It is to be noted that, to test the generalizability, we have compared our approach with similar 



%Medical images suffer from problems like noise and blurred boundaries, which makes it difficult to segment the region of interest using only the low level features. 

%Meanwhile, it is difficult to accurately predict boundaries using only the high level features which lack relevant spatial information of the image. U-Net solved this problem by combining low level and high level feature maps through skip connections.


%Another category of networks in the field of medical image segmentation are cascaded segmentation networks. The goal of such networks is predicting an initial coarse segmentation map and refining it with subsequent netowrks. Christ et al.~\cite{christ2016automatic} designed a cascaded network for liver and liver tumor segmentation. \ac{FCN} was used to predict segmentation map for liver which was further used in another \ac{FCN} for liver tumor segmentation. Feng et al.~\cite{feng2019automatic} improved the previous work by replacing the \ac{FCN}'s in the previous work by U-Net~\cite{ronneberger2015u}. Jha et al. proposed DoubleU-Net~\cite{jha2020doubleUNet} which used an initial U-Net with VGG-19~\cite{simonyan2014very} as the backbone to give an initial prediction of the target segmentation map and refined it using another variant of U-Net.

%This technique has been further used in mU-Net~\cite{seo2019modified}. %Chen et al.~\cite{chen2019feature} further devised an attention based feature fusion between the high and low level features in their proposed FED-Net. 

%Wang et al.~\cite{wang2019sclerasegnet} proposed ScleraSegNet which introduced an attention module in the bottleneck between encoder and the decoder sub-network. The conducted experiments by using channel,spatial and different combinations of the attention methods for medical image segmentation tasks and reported that channel wise attention gave the most effective performance. 

%Recurrent Neural Network(RNN) is used to model sequence of data and in the case of medical image segmentation it can be used to model the time dependence of image sequence. Alom et al.~\cite{alom2018recurrent} incorporated RNN in ResUnet~\cite{zhang2018road} to form RU-Net and R2U-Net. The RNN's allowed efficient feature accumulation with respect to different time-steps and formed stronger feature representations.


%Initially approaches towards the problem of medical image segmentation involved contour and shape based methods, region- and edge-based methods, deformable models, Gaussian mixture model fitting and clustering~\cite{petitjean2011review}~\cite{ghose2012survey}. Zhao et al.~\cite{yu2006medical} devised a mathematical morphological edge detection algorithm for lungs CT image. Lalonde et al.~\cite{lalonde2001fast} used pyramidal decomposition for large scale object tracking to guide a Hausdorff-based template matching for localization of the optic disk in low-resolution color fundus images. Tsai et al.~\cite{tsai2003shape} used a shape-based approach to curve evolution for segmentation of 2D cardiac \ac{MRI} and 3D prostate \ac{MRI}. Held et al.~\cite{held1997markov} used Markov random field for segmentation of brain \ac{MRI}. The advent of convolutional neural networks has disposed of the need of handcrafted features for medical image segmentation. The power of CNN's to successfully extract heirarchical features and its robustness in case of image noise, blur, low contrast make them a reliable solution for medical image segmentation.



% that are applied on feature maps and fused together to capture multi-resolution context without downscaling
%HRNet~\cite{Wang_2020} processes all the resolution streams in parallel, keeping the resolution representation for each resolution and performing the feature fusion across all resolution scales.
% Motivation
% In segmentation, fusing multi-resolution representations is computationally expensive and requires a large size dataset for efficient and effective training, which is not the case in most medical image segmentation applications.



evaluation metrics
%We have computed performance of our method and compared with SOTA methods using each of these metrics for all the datasets. 
% If \tp, \fp, \tn, and \fn are true positives, false positives, true negatives, and false negatives, respectively, the \ac{DSC}, \ac{IoU}, recall and precision is defined as:
% \begin{equation}{\label{eq:dsc}}
% \text{DSC} = 2 \times \frac{\tp} {\tp + \fp + \fn}
% \end{equation}
% %%
% \begin{equation}{\label{eq:iou}}
% \text{IoU} = \frac{\tp} {\tp + \fp + \fn}
% \end{equation}
% %
% \begin{equation}{\label{eq:recall}}
% \text{r} = \frac{\tp} {\tp + \fn}
% \end{equation}
% %
% \begin{equation}{\label{eq:precission}}
% \text{p} =\frac{\tp} {\tp + \fp}
% \end{equation}
%

%\multicolumn{5}{l}{{$^\dag$ Conditional generative adversarial network} \hspace{.1cm} $^\diamond${Data augmentation}}\\ 
	   %\multicolumn{5}{l}{$^\bullet$Fully convolutional network \hspace{.1cm} {$^\psi$ multi-scale patch-based}}
	   

% \subsection{Impact of Combined Loss}
% We also study the impact of the combination of \lbce and \ldcs used in \lcomb introduced in Section~\ref{section:loss_comp}. We train the the \sysname with \lcomb = \ldcs and then with \lcomb = \lbce and compare the results in Table~\ref{table:ablationstudy}. We notice that using dice loss and binary cross-entropy loss individually decreases the performance of proposed \sysname. While training, using an equal weighted combination of \lbce and \ldcs in \lcomb gives a 1.58\% increase in \ac{DSC}, 2.37\% increase in \ac{mIoU}, 2.48\% decrease in recall, 5.23\% increase in precision as compared to the scenario where \lcomb = \lbce.


% %
% \subsection{Absence of shape stream and deep supervision}
% To fully understand the contribution of MSRF sub-network, we remove the shape stream from the \sysname architecture during training and testing stages. We can observe from Table~\ref{table:ablationstudy}, 0.23\% decrease in \ac{DSC} and a 0.07\% fall in \ac{mIoU}, a 5.07\% decrease in precision while posting a 5.02\% increase in recall as compared to the original \sysname. Even though a small performance dip is noted, Our \sysname is capable of beating other \ac{SOTA} methods without the shape stream. Another experiment involved training \sysname while disabling deep supervision. Deep supervision provides better flow of gradients and regularization and disabling it causes a performance drop of 2.29\% \ac{DSC}, 4.65\% \ac{mIoU}, 1.45\% recall and 3.99\% precision as compared to the original \sysname with deep supervision.


%
% \subsubsection{Presence of a \ac{MSRF} sub-network}
% To verify the contribution of the \ac{MSRF} sub-network, we disable the entire  \ac{MSRF} sub-network from the full network while keeping each component of the network intact and train the model. From Table~\ref{table:ablationstudy}, we can observe that the \ac{DSC} drops by 4.46\%.  The performance degradation shows that the \ac{MSRF} sub-network contributes to the network. The combination of high- and low-level resolution feature representations of varying receptive fields extracted from the \ac{MSRF} sub-network was instrumental in improving the model's performance.

% \subsubsection{Scaling in \ac{MSRF} sub-network} The sub-network (SN) without scaling in Table~\ref{table:ablationstudy} demonstrates the influence of scaling factor $w$ in the network (refer Eq.~\ref{eq:5}). For this experiment, we do not scale the output of \ac{DSDF} by a constant while adding to the block's input. Again, a performance drop of 0.80\% in \ac{DSC} was observed when the features were not scaled. 
%
% \subsubsection{Multi-scale fusion in \sysname}
% We also ablate if multi-scale fusion was suitable for the entire network. SN without \ac{DSDF} refers to the removal of \ac{DSDF} with 2nd and 3rd scale inputs (also see Figure~\ref{fig:smfrdbblock}, where middle \ac{DSDF} blocks represent them, i.e., layer three and layer five are removed). Table~\ref{table:ablationstudy} shows the result when global multi-scale fusion is absent from the network. As a result, we observe a 2.04\% performance drop in \ac{DSC}. Therefore, it is noticeable that the multi-scale fusion used in the \ac{MSRF} sub-network in~\sysname architecture improves performance.
%
% \subsubsection{Impact of Number of \ac{DSDF} blocks used}
% To study the impact of the number of \ac{DSDF} blocks on the segmentation performance, we reduced the number of \ac{DSDF} layers from six (ours) to three, i.e., only red rectangular block in Figure~\ref{fig:smfrdbblock} b is used. Even though this enables us to exchange global multi-scale feature representations, our results in Table~\ref{table:ablationstudy} show that reducing the number of \ac{DSDF} blocks degrades the performance of the network by 2.31\%. 
%
% \subsubsection{Shape or boundaries prediction} 
% We have trained the proposed \sysname and a variant of \sysname to analyze the impact of the \ac{MSRF} sub-network on the shape stream. The variant model uses the shape stream before the \ac{MSRF} sub-network using only the features captured by the encoder. The \ac{MSRF} sub-network is placed after the shape-stream in the \sysname keeping the number of parameters same for both the models. The qualitative results (Figure~\ref{fig:shapestream}) show that the \sysname can define more precise and more spatially accurate boundaries than the variant model. The variant model fails to recognize the boundaries of the target structure as it is deprived of the multi-scale features extracted by the \ac{MSRF} sub-network. This validates our choice of putting the MSRF sub-network before the shape stream block.
%
% \subsection{Impact of scaling coefficient w}
% We train the proposed \sysname using different scaling values of $w$ introduced in Equation~\ref{eq:5}. The aim is to understand the impact different scaling values have on the performance of \sysname. We can observe from Figure~\ref{fig:hyperparamw} that initially the \ac{DSC} is lower and drops the lowest when $w=0.3$. Highest \ac{DSC} is achieved when $w$ is set to $0.4$, further increasing $w$ decreases \ac{DSC}.   


% TODO: Say something about how you would improve, e.g. network limitation and what you will do next (just briefly)
%

% \section{Generalization}
%In medical imaging, generalization is the ability of the algorithm trained on specific interventions in specific hospitals that should be able to generalize over other interventions or hospitals~\cite{ross2020robust}.   Table~\ref{tab:generalizationkvasir} and Table~\ref{tab:generalizationcvc} present the generalizability results. 
%
% \subsection{Generalizibility results on CVC-ClinicDB}
% Table~\ref{tab:generalizationkvasir} shows the generalizability results of the \sysname model trained on Kvasir-SEG and tested on CVC-ClinicDB. Despite using two datasets acquired using two different imaging protocols, \sysname obtained an acceptable \ac{DSC} of 0.7921, \ac{mIoU} of 0.6498, recall of 0.9001, and precision of 0.7000. We observe that our \sysname performs better than other \ac{SOTA} methods in terms of \ac{DSC}. HRNetV2-W48~\cite{Wang_2020} obtained a competitive \ac{DSC} of 0.7901. 
% %
% \subsection{Generalizibility results on Kvasir-SEG}
% Similarly, we present the results of the models trained on CVC-ClinicDB and tested on Kvasir-SEG in Table~\ref{tab:generalizationcvc}. We report that our model achieves a \ac{DSC} of 0.7575, \ac{mIoU} of 0.6337, recall of 0.7197 and precision of 0.8414, which outperforms other \ac{SOTA} methods in all presented metrics. The second best performing method is UNet++~\cite{zhou2019unet++} with \ac{DSC} of 0.6783, and \ac{mIoU} of 0.5494. Our method outperforms UNet++ by 7.92\% in \ac{DSC} and 8.43\% in \ac{mIoU}. 
%
% \subsection{Ablation study}
% {\label{sec:ablationStudy}}

%%%
%
%


% TODO This is nicely written. I will have second look at the end.
%{\color{red}While U-Net~\cite{ronneberger2015u} uses skip-connections for feature fusion, the resulting combination of features suffer from semantic gap since they combine low level features of the encoder and high level features of the decoder. U-Net++\cite{zhou2019unet++} performs low to high feature fusion to overcome this problem, but high to low feature fusion remains lacking. Deeplabv3+~\cite{chen2018encoder} fuses the pyramid features while forgoing the high resolution representations. HR-Net builds upon the multi-scale feature fusion process by adding repeated feature fusion while maintaining high resolution representation. Their fusion modules are computationally expensive and} {\color{red}informative low level features are also lost during the segmentation process. Perhaps, these disadvantages consequently result in Deeplabv3+~\cite{chen2018encoder} and HRNetV2~\cite{wang2020deep} to perform considerably worse on the 2018 Data Science Bowl challenge where finer segmentation maps were required for a high \ac{DSC} score. While the proposed \sysname uses \ac{DSDF} blocks arranged as described in Algorithm~\ref{alg:algo1} attains global multi-scale fusion while increasing the frequency of multi-scale fusion while reporting a lower computational complexity than HRNetV2~\cite{wang2020deep}. Additionally our \sysname is able to retain relevant high- and low level features to form accurate segmentation maps.} 
% Start from Table VI - Table VII: Generalisation
% motivation about it and then observations
%
%

% TODO: First motivate why one needs to see generalisation ability and second why this is an important comparison : DONE


%
% \subsubsection{Generalisation}
% \label{section:general}
% \subsubsection{Ablation study}{\label{sec:ablationStudy}}
% Few lines describtion
%Table ref and results (values) (least or highest, ) --> do not discuss!!
%As it can be observed that our proposed network outperforms all the ablated networks with DSC of $0.9217$ ±$ 0.168$ and  $0.9194$ ±$ 0.1779$ with and without using shape-stream, respectively. MSRF sub-network without scaling reports a \ac{DSC} of 0.9137 ± 0.1772. The removal of triple attention mechanism from the decoder blocks MSRF sub-network without scaling reports a \ac{DSC} of 0.9137 ± 0.1772. Further performance improvement can be seen with addition of sub-network for both without scaling (value) and without DSDF across 2 and 3 scales (value). Our ablation on removing deep supervision resulted in a lower \ac{DSC} of $0.8988$$ ±$ 0.2060. A similar trend was observed for other metrics.   



 %In each quantitative comparison we report the \ac{DSC}, \ac{mIoU}, recall and precision along with standard deviation for each metric. The \ac{DSC} of each method are compared against our \sysname using paired t-test and the p-values are reported. Each table compares the number of parameters and \ac{FPS} achieved for each method. 

%% TODO: write what readers will find here (2-3 sentences)
%
% \subsection{Results}


%
%The implementation details on the data augmentation and proposed model can be found in the \textbf{Supplementary materials}.

% The qualitative comparison of the ground truth and the predicted mask for the corresponding input image is shown. % (from left to right: Kvasir-SEG~\cite{jha2020kvasir}, CVC-ClinicDB~\cite{bernal2015wm}, 2018 Data Science Bowl~\cite{caicedo2019nucleus}, and ISIC-2018~\cite{codella2018skin,tschandl2018ham10000}) 

%From Table~\ref{table:ablationstudy}, we can observe that the mean \ac{DSC} drops by 4.46\% when we remove the \ac{MSRF} sub-network from our p.
%

%When both precision and recall are taken into consideration, MSRF-Net achieves a higher score than the individual scores of combinations of ResUNet++ and conditional random field~\cite{jha2021comprehensive} and  DoubleUNet~\cite{jha2020doubleu}.
%
\subsubsection{Comparison on Kvasir-SEG}

\begin{table*}[!t]
{\color{red}
\centering
%\scriptsize
\footnotesize
\caption{Result comparison on the Kvasir-SEG. We have not computed paired t-test (p values) for the same network (MSRF-Net)\textsuperscript{$R_{2,4}$}\textsuperscript{$R_{3,3}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,6}$}\textsuperscript{$R_{3,8}$}}
\begin{tabular}{@{}l|l|l|l|l|l|l|l@{}}
\toprule
\textbf{Method} & \textbf{DSC} & \textbf{p-values} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision} & \textbf{Parameters} & \textbf{FPS}\\ 
\hline
\hline
U-Net~\cite{ronneberger2015u} & 0.8629 ± 0.2334 & 1.559e-02 & 0.8176 ± 0.2465 & 0.9094 ± 0.2216 &0.8901 ± 0.2313  & 7.11M & 41.04  \\ \hline
U-Net++~\cite{zhou2019unet++} & 0.7475 ± 0.2664 & 4.363e-10 & 0.6313 ± 0.2788 & 0.6865 ± 0.2888 & 0.8871 ± 0.2689 & 9.04M & 30.67 \\ \hline
%ResUNet-mod~\cite{zhang2018residual} & 0.7909  & 0.4287 & 0.6909 & 0.8713\\ \hline
ResUNet++~\cite{jha2019resunet++} & 0.8189 ± 0.2652 &6.518e-06 & 0.7918 ± 0.2819 & 0.8372 ± 0.2751 & 0.9255 ± 0.2545 & 4.07M & 15.92\\ \hline
%SFA (MICC AI'19)~\cite{fang2019selective} & 0.7230 & 0.6110 & -   & -  \\ \hline
%ColonSegNet~\cite{jha2020real}& 0.8206 & 0.7239 & 0.8496 & 0.8435 \\ \hline

Deeplabv3+( Xception)~\cite{chen2018encoder} & 0.8965 ± 0.2072 & 3.660e-01 & 0.8575 ± 0.2290  & 0.8984 ± 0.2099  & 0.9496 ± 0.1801 & 41.25M & 49.11 \\ \hline

Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.8656 ± 0.2032 & 1.409e-04 & 0.8186 ± 0.2222 & 0.8808 ± 0.2105 & 0.9205 ± 0.1980 & 2.14M & 118.50\\ \hline


{DoubleUNet}~\cite{jha2020doubleu} &0.8699 ± 0.1585 & 8.109e-05 & {0.8166} ± {0.1933} &{0.9039} ± 0.1810 & 0.8942 ± 0.1586 & 29.29M & 7.46 \\ \hline

HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.8179 ± 0.2067 & 4.844e-06 & 0.7470 ± 0.2622  & 0.8016 ± 0.2681 & 0.8696 ± 0.2494 & 26.20M & 52.68 \\ \hline

HRNetV2-W48~\cite{Wang_2020} & 0.8896 ± 0.1200 & 5.935e-04 & 0.8262 ± 0.1856 & 0.8973 ± 0.1719 & 0.9056 ± 0.1492 & 65.84M & 29.79 \\ \hline


ColonSegNet~\cite{jha2020real} & 0.8203 ± 0.2295 & 8.692e-07 & 0.7435 ± 0.2539 & 0.8124 ± 0.2494  & 0.8832 ± 0.1985 & 5.01M & 24.26 \\ \hline

DDANet~\cite{tomar2020ddanet}& 0.8915 ± 0.1880 & 2.558e-02 & 0.8393 ± 0.2126 & 0.8927 ± 0.2093 & 0.9213 ± 0.1604 & 6.83M & 7.76\\ \hline

ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}&0.7965 ± 0.2707 & 1.721e-06 &0.8250 ±0.2832 &0.8119 ± 0.2803  &0.8045 ± 0.2638 & 4.02M & 15.12 \\ \hline

PraNet~\cite{fan2020pranet}  & 0.9078 ± 0.1543 & 3.693e-01 & 0.8561 ± 0.1823 & 0.9034 ± 0.1719 & 0.9352 ± 0.1358 & 32.54M & 48.25  \\ \hline

UACANet-S~\cite{kim2021uacanet} & 0.8800 ± 0.2042 & 3.871e-04 & 0.8250 ± 0.2215 & 0.8701 ± 0.2136 & 0.9229 ± 0.1758 & 26.90M & 32.58 \\ \hline

UACANet-L~\cite{kim2021uacanet} & 0.9014 ± 0.1878 & 4.878e-01 & 0.8555 ± 0.2098 & 0.8897 ± 0.2148 & 0.9381 ± 0.1458 & 69.15M & 28.40 \\ \hline

\sysname(ours) & \textbf{0.9217} ± 0.1685 & - & \textbf{0.8914} ± 0.1938 & \textbf{0.9198} ± 0.1919 & \textbf{0.9666} ± 0.1379 & 18.38M & 14.38\\ \hline
\bottomrule
\end{tabular}
\label{tab:result1}}
\end{table*}

\subsubsection{Comparison on CVC-ClinicDB}
\begin{table*}[!t]
{\color{red}
\centering
%\scriptsize
\footnotesize
\caption{Result comparison on the CVC-ClinicDB\textsuperscript{$R_{2,7}$}\textsuperscript{$R_{3,3}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,6}$}\textsuperscript{$R_{3,8}$}}
\label{tab:result2}
\begin{tabular}{@{}l|l|l|l|l|l|l|l@{}}
\toprule
\textbf{Method} &\textbf{DSC}& \textbf{P-values}   &\textbf{mIoU} &\textbf{Recall} &\textbf{Precision}& \textbf{Parameters} & \textbf{FPS} \\
\hline
\hline
%FCN~\cite{li2017colorectal} &-&-&0.7732 & 0.8999\\ \hline
% CNN~\cite{nguyen2018colorectal} &0.8700 & - & - & -\\ \hline
% SegNet~\cite{wang2018development} & -  & - & 0.8824 & -     \\ \hline
% MSPB$^\psi$CNN~\cite{banik2020multi}& 0.8130 & - & 0.7860 &  0.8090\\ \hline
% MultiResUNet$^\diamond$~\cite{ibtehaz2020multiresunet} & -  & 0.8497 & - & -  \\ \hline
% CGAN$^\dag$~\cite{poomeshwaran2019polyp} & 0.8848  & 0.8127 &-  &  - \\ \hline

U-Net~\cite{ronneberger2015u}  & 0.9145 ± 0.1390 & 1.000e+00$^\star$ & 0.8654 ± 0.1514 &0.9178 ± 0.1309 &0.9381 ± 0.1594 & 7.11M & 22.84    \\ \hline

U-Net++~\cite{zhou2019unet++} & 0.8453 ± 0.1516 & 6.400e-04 & 0.7559 ± 0.1188 & 0.8917 ± 0.2594 & 0.8323 ± 0.2713 & 9.04M & 17.60 \\ \hline

ResUNet++$^\diamond$~\cite{jha2019resunet++} & 0.9075 ± 0.1455 & 1.000e+00$^\star$ & 0.8587 ± 0.1616 & 0.9156 ± 0.1372 & 0.9325 ± 0.1593 & 4.07M & 15.71 \\ \hline

Deeplabv3+ (Xception)~\cite{chen2018encoder} & 0.8897 ± 0.1895 & 6.723e-01 & 0.8706 ± 0.2036 & 0.9251 ± 0.1965 & 0.9366 ± 0.1621 & 41.25M & 29.08 \\\hline

Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.8985 ± 0.1385 & 2.838e-01 & 0.8588 ± 0.1544 & 0.9160 ± 0.1562 & 0.9287 ± 0.1378 & 2.14M & 55.68 \\ \hline

DoubleU-Net~\cite{jha2020doubleu} & 0.9272 ± 0.1761  & 1.000e+00$^\star$ & 0.8889 ± 0.1896 & 0.9395 ± 0.1800 & \textbf{0.9592} ± 0.1609 &  29.29M & 7.46 \\ \hline

\textsuperscript{$R_{3,7}$}HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.9073 ± 0.1158 & 1.000e+00$^\star$ & 0.8457 ± 0.1477 & 0.9137 ± 0.1293 & 0.9191 ± 0.1060 & 26.20M & 57.47 \\ \hline 

\textsuperscript{$R_{3,7}$}HRNetV2-W48~\cite{Wang_2020} & 0.9244 ± 0.1280 & 1.000e+00$^\star$ & 0.8747 ± 0.1332 & 0.9234 ± 0.1356 & 0.9296 ± 0.1318 & 65.84M & 29.76 \\ \hline

ColonSegNet~\cite{jha2020real} & 0.9132 ± 0.1416 & 1.000e+00$^\star$ & 0.8600 ± 0.1585 & 0.9072 ± 0.1564  & 0.9292 ± 0.1393 & 5.01M & 7.98 \\ \hline

DDANet~\cite{tomar2020ddanet} & 0.9233 ± 0.1339 & 1.000e+00$^\star$ & 0.8747 ± 0.1438 & 0.9271 ± 0.1285 & 0.9259 ± 0.1495 & 6.83M & 58.15 \\ \hline
ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}&0.8815 ± 0.1507 & 1.102e-01 &0.8899 ± 0.1685 &0.8970 ± 0.1581  &0.8674 ± 0.1605 & 4.02M & 8.55 \\ \hline

PraNet~\cite{fan2020pranet}  & 0.9072 ± 0.1695 & 1.000e+00$^\star$ & 0.8575 ± 0.1823 & 0.9227 ± 0.1657 & 0.9134 ± 0.1614 & 32.54M & 47.92 \\ \hline

UACANet-S~\cite{kim2021uacanet} & 0.9190 ± 0.1426 & 1.000e+00$^\star$ & 0.8700 ± 0.1556 & 0.9285 ± 0.1356 & 0.9201 ± 0.1574 & 26.90M & 31.79 \\ \hline

UACANet-L~\cite{kim2021uacanet}& 0.9098 ± 0.1829 & 1.000e+00$^\star$ & 0.8649 ± 0.1872 & 0.9174 ± 0.1772 & 0.9114 ± 0.1950  & 69.15M & 32.81 \\ \hline

\sysname (Ours) & \textbf{0.9420} ± 0.0804 & - & \textbf{0.9043} ± 0.1009 & \textbf{0.9567} ± 0.0620 & 0.9427 ± 0.0994 & 18.38M & 12.50  \\
\hline
\bottomrule
 \multicolumn{6}{l}{$^\star$ \textit{large improvements were still observed for some samples with consistent Dice scores (also see standard deviation) for \sysname} \hspace{.1cm}}
\end{tabular}}
\end{table*}

\begin{table*}[!t]
{\color{red}
\centering

\scriptsize
%\footnotesize
\caption{Results on the 2018 Data Science Bowl\textsuperscript{$R_{2,7}$}\textsuperscript{$R_{3,3}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,6}$}\textsuperscript{$R_{3,8}$}}
\label{tab:result3}
\begin{tabular}{@{}l|l|l|l|l|l|l|l@{}}
\toprule
\textbf{Method} & \textbf{DSC} & \textbf{P-values}& \textbf{mIoU}& \textbf{Recall} & \textbf{Precision} & \textbf{Parameters} & \textbf{FPS}\\ 
\hline
\hline
U-Net~\cite{ronneberger2015u} & 0.9080 ± 0.0638 & 1.308e-03 & 0.8314 ± 0.1019 & 0.9029 ± 0.0981 & 0.9130 ± 0.0719  & 7.11M & 25.02    \\ \hline
U-Net++~\cite{zhou2019unet++}  & 0.7705 ± 0.3010 & 4.832e-04 & 0.5265 ± 0.3078 & 0.7159 ± 0.3171& 0.6657 ± 0.2745 & 9.04M & 21.86\\ \hline
ResUNet++$^\diamond$~\cite{jha2019resunet++} & 0.9098 ± 0.0797 & 2.420e-01 & 0.8370 ± 0.1154 & 0.9169 ± 0.0947 & 0.9057 ± 0.0853 & 4.07M & 19.81 \\ \hline
Deeplabv3+ (Xception)~\cite{chen2018encoder} & 0.8857 ± 0.1674 & 4.641e-01 & 0.8367 ± 0.1702 & 0.9141 ± 0.1751 & 0.9081 ± 0.1689 & 41.25M & 16.20 \\\hline
Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.8239 ± 0.1613 & 1.044e-06 & 0.7402 ± 0.1618 & 0.8896 ± 0.1720 & 0.8151 ±  0.1657 & 2.14M & 23.70 \\ \hline
DoubleUNet~\cite{jha2020doubleu} & 0.9109 ± 0.0876 & 8.929e-02 & 0.8429 ± 0.1109 &  0.9278 ± 0.0962 & 0.9020 ± 0.0997 & 29.29M & 7.47 \\ \hline
HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.8495 ± 0.3267 & 4.978e-04 & 0.7585 ± 0.1521 & 0.8640 ± 0.1659 & 0.8398 ± 0.1602 & 26.20M & 58.03  \\ \hline 
HRNetV2-W48~\cite{Wang_2020} & 0.8488 ± 0.1470 & 8.460e-05 & 0.7588 ± 0.1499 & 0.8359 ± 0.1618 & 0.8913 ± 0.0550 & 65.84M & 29.41  \\ \hline
ColonSegNet~\cite{jha2020real} & 0.9197 ± 0.0605 & 6.433e-01 & 0.8466 ± 0.0953 & 0.9153 ± 0.0917  & \textbf{0.9312} ± 0.0532 & 5.01M & 16.56  \\ \hline
DDANet~\cite{tomar2020ddanet} & 0.9182 ± 0.0684 & 5.922e-01 & 0.8452 ± 0.1037  & 0.9139 ± 0.0964 & 0.9289 ± 0.0575 & 6.83M & 19.02 \\ \hline
ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}& 0.7806 ± 0.2223 & 6.971e-06 & 0.7322 ± 0.2386 & 0.7534 ± 0.2558 & 0.6308 ± 0.1752 & 4.02M & 72.78 \\ \hline
PraNet~\cite{fan2020pranet}  &0.8751 ± 0.0871 & 1.553e-07 & 0.7868 ± 0.1169 & 0.9182 ± 0.0736 & 0.8438 ± 0.1138 & 32.54M & 11.88 \\ \hline
UACANet-S~\cite{kim2021uacanet} &0.8687 ± 0.0913 & 2.940e-08 & 0.7774 ± 0.1208 & 0.9092 ± 0.0960& 0.8385 ± 0.1115 & 26.90M & 28.08 \\ \hline
UACANet-L~\cite{kim2021uacanet}&0.8688 ± 0.0999 & 8.975e-07 &0.7791 ± 0.1283 &0.9061 ± 0.1057 & 0.8414 ± 0.1141 & 69.15M & 32.26 \\ \hline
\sysname (Ours)  &\textbf{0.9224} ± 0.0538 & - &\textbf{0.8534} ± 0.0870  & \textbf{0.9402} ± 0.0734  & 0.9022 ± 0.0601 & 18.38M & 6.84 \\ \hline 
\bottomrule
\end{tabular}}

\end{table*}
%
\begin{table*}[!t]
{\color{red}
\centering
\scriptsize
%\footnotesize
\caption{Results on the ISIC-2018 skin lesion segmentation challenge\textsuperscript{$R_{2,7}$}\textsuperscript{$R_{3,3}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,6}$}\textsuperscript{$R_{3,8}$}}
\label{tab:result4}
\begin{tabular}{@{}l|l|l|l|l|l|l|l@{}}
\toprule
\textbf{Method} & \textbf{DSC} & \textbf{P-values} & \textbf{mIoU}& \textbf{Recall} & \textbf{Precision}& \textbf{Parameters} & \textbf{FPS}\\  \hline
\hline
\hline
U-Net~\cite{ronneberger2015u} & 0.8554 ± 0.1848 & 1.315e-02 & 0.7847 ± 0.2094 & 0.8204 ± 0.2186 & \textbf{0.9474} ± 0.1296 & 7.11M & 79.43 \\ \hline
U-Net++~\cite{zhou2019unet++}  & 0.8094 ± 0.2261 & 6.336e-08 & 0.7288 ± 0.2452 & 0.7866 ±  0.2369 & 0.9084 ± 0.2222 & 9.04M & 60.44 \\ \hline
ResUNet++$^\diamond$~\cite{jha2019resunet++} & 0.8557 ± 0.2014 & 1.813e-02 & 0.8135 ± 0.2210 & 0.8801 ± 0.2320 & 0.8676 ± 0.1562 & 4.07M & 40.93 \\ \hline
Deeplabv3+ (Xception)~\cite{chen2018encoder} & 0.8772 ± 0.1465 & 4.314e-02 & 0.8128 ± 0.1806 & 0.8681 ± 0.1792 & 0.9272 ± 0.13602 & 41.25M & 43.53 \\\hline
Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.8781 ± 0.1371 & 9.503e-02 & 0.8236 ± 0.1711 & 0.8830 ± 0.1725 & 0.9244 ± 0.1317 & 2.14M & 61.10 \\ \hline
HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.8561 ± 0.3696 & 8.780e-03 & 0.7821 ± 0.2091 & 0.8556 ± 0.2029 & 0.8974 ± 0.1862 & 26.20M & 57.47 \\ \hline 
\textsuperscript{$R_{3,7}$}HRNetV2-W48~\cite{Wang_2020} & 0.8667 ± 0.2453 & 4.270e-02 & 0.8109 ± 0.2630 & 0.8584 ± 0.2936 & 0.9155 ± 0.2755 & 65.84M & 28.54 \\ \hline

\textsuperscript{$R_{3,8}$}DoubleU-Net~\cite{jha2020doubleu} &{\textbf{0.8938}} ± 0.1362 & 1.000e+00 & {0.8212} ± {0.1659} & 0.8780 ± {0.1573} & {0.9459} ± {0.1353} & 29.29M & {7.46}  \\ \hline

ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}& 0.8688 ± 0.1719 & 1.813e-02 & 0.8209 ± 0.1971 & 0.8826 ± 0.2063 & 0.8736 ± 0.1540 & 4.02M & 79.11 \\ \hline
MSRF-Net (Ours) & 0.8824 ± 0.1602 & - &  \textbf{0.8373} ± 0.1818 &\textbf{0.8893} ± 0.1889 & 0.9348 ± 0.1488 & 18.38M & 16.10 \\ \hline   
\bottomrule
\end{tabular}}

\end{table*}
\begin{table*} [!t]
{\color{red}
\centering
\scriptsize
%\footnotesize
\caption{Generalizability results of the models trained on Kvasir-SEG and tested on  CVC-ClinicDB\textsuperscript{$R_{2,7}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,8}$}}
\label{tab:generalizationkvasir}
%
\begin{tabular}{l|r|r|r|r|r|r}
\toprule
\textbf{Method} & \textbf{DSC} & \textbf{mIoU}& \textbf{Recall} & \textbf{Precision} & \textbf{Parameters} & \textbf{FPS} \\\hline
U-Net~\cite{ronneberger2015u} & 0.7172 ± 0.2911 & 0.6133 ± 0.2870 & 0.7255 ± 0.3246 & \textbf{0.7986} ± 0.2775 & 7.11M & 24.15\\ \hline

U-Net++~\cite{zhou2019unet++}  & 0.4265 ± 0.3922  & 0.3345 ± 0.3518 & 0.3939 ± 0.4480 & 0.6894 ± 0.4111   & 9.04M & 21.18     \\ \hline
ResUNet++$^\diamond$~\cite{jha2019resunet++} & 0.5560 ± 0.3436 & 0.4542 ± 0.3174 & 0.5795 ± 0.3896 & 0.6775 ± 0.3579 & 4.07M & 8.84 \\ \hline

Deeplabv3+ (Xception)~\cite{chen2018encoder} & 0.6509 ± 0.3172 & 0.5385 ± 0.3174 & 0.6251 ± 0.3621 & 0.7947 ± 0.3175 & 41.25M &  27.24\\\hline

Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.6303 ± 0.2740 & 0.4825 ± 0.2716 & 0.5957 ± 0.3391 & 0.7173 ± 0.2730 & 2.10M & 73.64\\ \hline

HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.6428 ± 0.3003 & 0.5513 ± 0.3213 & 0.6811 ± 0.3753 & 0.7253 ± 0.3191 & 26.20M & 57.32 \\ \hline 

HRNetV2-W48~\cite{Wang_2020} & 0.7901 ± 0.2280 & \textbf{0.6953} ± 0.2455  & 0.8796 ± 0.1746 & 0.7694 ± 0.2642 & 65.84M & 29.24\\ \hline

ColonSegNet~\cite{jha2020real} & 0.6895 ± 0.2716 & 0.5813 ± 0.2754 & 0.7862 ± 0.2965  & 0.7177 ± 0.2897 & 5.01M & 17.01\\ \hline

ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}& 0.6502 ± 0.3381 & 0.7417 ± 0.3147 & 0.7047 ± 0.3631 & 0.6277 ± 0.3392 & 4.02M & 80.31  \\ \hline

PraNet~\cite{fan2020pranet}  & 0.7225 ± 0.2931 & 0.6328 ± 0.3028 & 0.7531 ± 0.3390 & 0.7888 ± 0.2953 & 32.54M & 30.91  \\ \hline

UACANet-S~\cite{kim2021uacanet} & 0.5683 ± 0.3799 & 0.4907 ± 0.3631 & 0.5792 ± 0.4101 & 0.7095 ± 0.3833 & 26.90M & 32.61 \\ \hline

UACANet-L~\cite{kim2021uacanet}& 0.5589 ± 0.3899  & 0.4849 ± 0.3689 & 0.5800 ± 0.4276 & 0.6775 ± 0.3906 & 69.15M & 32.20 \\ \hline

MSRF-Net (Ours) & \textbf{0.7921} ± 0.2564 & 0.6498 ± 0.2729 & \textbf{0.9001} ± 0.2980 & 0.7000 ± 0.1572 & 18.38M & 10.94\\ \hline   
\bottomrule
\end{tabular}}

\end{table*}
%
%
\begin{table*}[!t]
{\color{red}
\centering
\scriptsize
\caption{Generalizability results of the models trained on CVC-ClinicDB and tested on Kvasir-SEG\textsuperscript{$R_{2,7}$}\textsuperscript{$R_{3,4}$}\textsuperscript{$R_{3,8}$}}
\label{tab:generalizationcvc}
\begin{tabular}{l|r|r|r|r|r|r}
\toprule
\textbf{Method} & \textbf{DSC} & \textbf{mIoU}& \textbf{Recall} & \textbf{Precision}& \textbf{Parameters} & \textbf{FPS}  \\ 
\hline
\hline
U-Net~\cite{ronneberger2015u} & 0.6222 ± 0.2595 & 0.4588 ± 0.2609 & 0.5129 ± 0.1766 & 0.8133 ± 0.3059 & 7.11M & 35.18\\ \hline

U-Net++~\cite{zhou2019unet++}  & 0.5926 ± 0.2363  & 0.4564 ± 0.2321 & 0.7352 ± 0.2368 & 0.5462 ± 0.2902  & 9.04M & 16.85      \\ \hline

ResUNet++$^\diamond$~\cite{jha2019resunet++} & 0.5147 ± 0.3138 & 0.4082 ± 0.2940 & 0.7181 ± 0.3331 & 0.4860 ± 0.3530 & 4.07M & 25.86 \\ \hline

\textsuperscript{$R_{3,7}$}HRNetV2-W18-Smallv2~\cite{Wang_2020} & 0.7012 ± 0.0680 & 0.6009 ± 0.2889 & 0.7184 ± 0.3021 & 0.7666 ± 0.2863  & 26.20M & {57.89} \\ \hline 

\textsuperscript{$R_{3,7}$}HRNetV2-W48~\cite{Wang_2020} & 0.7404 ± 0.1489 & 0.6233 ± 0.2834 & 0.7293 ± 0.2830 & \textbf{0.8511} ± 0.2563 & 65.84M & 29.80\\ \hline

Deeplabv3+ (Xception)~\cite{chen2018encoder} & 0.6746 ± 0.2746 & 0.5327 ± 0.2788 & 0.7757 ± 0.2967 & 0.6296 ± 0.2699 & 41.25M & 39.62\\\hline

Deeplabv3+ (Mobilenet)~\cite{chen2018encoder} & 0.6474 ± 0.2634 & 0.5098 ± 0.2653 & 0.6632 ± 0.2611 & 0.6878 ± 0.2916 & 2.10M & 78.63\\ \hline

ColonSegNet~\cite{jha2020real} & 0.6324 ± 0.2772 & 0.5183 ± 0.2830 & 0.6112 ± 0.3058  & 0.7897 ± 0.2731 & 5.01M & 7.92 \\ \hline

ResUNet++ + CRF$^\diamond$~\cite{jha2021comprehensive}& 0.4200 ± 0.3150 & 0.6096 ± 0.2770 & 0.3782 ± 0.3132 & 0.6711 ± 0.4004 & 4.02M & 46.98  \\ \hline

PraNet~\cite{fan2020pranet}  & 0.7293 ± 0.3004 & 0.6262 ± 0.3128 & \textbf{0.8007} ± 0.2675 & 0.7623 ± 0.3243 & 32.54M & 49.61  \\ \hline
UACANet-S~\cite{kim2021uacanet} & 0.6945 ± 0.2634 & 0.5894 ± 0.2911 & 0.7692 ± 0.2424 & 0.7377 ± 0.3119 & 26.90M & 32.89 \\ \hline
UACANet-L~\cite{kim2021uacanet}& 0.7312 ± 0.2724  & 0.6383 ± 0.2961 & 0.7417 ± 0.2803 & 0.8314 ± 0.2627 & 69.15M & 32.73 \\ \hline

MSRF-Net (Ours) &  \textbf{0.7575} ± 0.2643 & \textbf{0.6337} ± 0.2815 &0.7197 ± 0.2775 &0.8414 ± 0.2731 & 18.38M & 16.24\\ \hline   
\bottomrule
\end{tabular}}

\end{table*}
%

\begin{table*}
\color{red}
\centering
\caption{Ablation study of \sysname on the Kvasir-SEG}
\label{table:ablationstudy}
\scriptsize
\begin{center}
{\textsuperscript{$R_{2,7}$}
	\begin{tabular}{@{}l|r|r|r|r|r|r@{}} 
		\toprule
		 \textbf{Experiment description} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision} & \textbf{Parameters} & \textbf{FPS} \\ %\hline
		 \hline
		 \hline
		 \sysname(ours) & \textbf{0.9217 ± 0.1685} & \textbf{0.8914} ± 0.1938 & 0.9198 ± 0.1919 & \textbf{0.9666} ± 0.1379 & 18.38M & 16.24\\ \hline
		 Without sub-network &0.8771 ± 0.2062 &0.8103 ± 0.2400 & 0.8911 ± 0.1742 & 0.8993 ± 0.2172 & 2.66M & 32.64 \\ \hline
		 Sub-network without scaling &0.9137 ± 0.1772 &0.8898 ± 0.2013 &0.9625 ± 0.1932 &0.9218 ± 0.1484 & 18.38M & 8.92 \\ \hline
		 Sub-network without DSDF$^\dag$ & 0.9013 ± 0.2111 & 0.8782 ± 0.2329 & 0.9460 ± 0.2098 & 0.9246 ± 0.2068 & 17.24M & 17.28  \\\hline
		 Subset of the sub-network & 0.8986 ± 0.1997 & 0.8570 ± 0.1262 & 0.9228 ± 0.2879 & 0.9232 ± 0.2666 & 8.67M & 13.10  \\ \hline
		 Without deep supervision & 0.8988 ± 0.2060 & 0.8449 ± 0.2313 & 0.9053 ± 0.1795 & 0.9267 ± 0.2152 & 18.38M & 16.58 \\ \hline
		 Without decoder block & 0.9067 ± 0.1834 & 0.8691 ± 0.2080 & 0.9143 ±  0.1875 & 0.9461 ± 0.1807 &17.41M & 16.90 \\ \hline
		 Without shape stream & 0.9194 ± 0.1779 & 0.8907 ± 0.1984 & \textbf{0.9700} ± 0.1976 & 0.9159 ± 0.1348 & 18.37M & 17.19\\
		 		 
		 \hline
		 MSRF-Net with \lcomb = \ldcs & 0.8861 ± 0.2192 & 0.8446 ± 0.2389 & 0.9139 ± 0.2078 & 0.9176 ± 0.2003 & 18.38M & 16.18\\ \hline
		 MSRF-Net with \lcomb = \lbce & 0.9059 ± 0.1859 & 0.8677 ± 0.2116 & 0.9446 ± 0.1938 & 0.9143 ± 0.17000 & 18.38M & 16.11\\ \hline
		 \bottomrule
		 \multicolumn{5}{l}{{$^\dag$(across 2,3 scale)} \hspace{.1cm}}\\
		 
	\end{tabular}}
\end{center}
\end{table*}



%Methods based on convolutional neural networks have improved the performance of biomedical image segmentation. However, most of these methods cannot efficiently segment objects of variable sizes and train on small and biased datasets, which are common in biomedical use cases. While methods exist that incorporate multi-scale fusion approaches to address the challenges arising with variable sizes, they usually use complex models that are more suitable for general semantic segmentation computer vision problems. In this paper, we propose a novel architecture called \sysname, which is specially designed for medical image segmentation tasks. The proposed \sysname is able to exchange multi-scale features of varying receptive fields using a dual-scale dense fusion block (DSDF). Our DSDF block can exchange information rigorously across two different resolution scales, and our MSRF sub-network uses multiple DSDF blocks in sequence to perform multi-scale fusion. This allows the preservation of resolution, improved information flow, and propagation of both high- and low-level features to obtain accurate segmentation maps. The proposed \sysname allows to capture object variabilities and provides improved results on different biomedical datasets. Extensive experiments on \sysname demonstrate that the proposed method outperforms most of the cutting-edge medical image segmentation state-of-the-art methods. We achieve the highest \ac{DSC} of 0.9217, 0.9420 and 0.9224 on Kvasir-SEG, CVC-ClinicDB and 2018 Data Science Bowl 2018 dataset. We further conducted generalizability tests and achieved the highest \ac{DSC} of 0.7921 and 0.7575 on unseen CVC-ClinicDB and Kvasir-SEG, respectively. \sysname advances the performance on four publicly available datasets and is more generalizable as compared to state-of-the-art methods. 
%{\color{red}\textsuperscript{$R_{4,3}$}In this paper, we propose a novel medical image segmentation architecture, called \emph{\sysname}, which aims to overcome the above limitations. Our proposed \sysname maintains high-resolution representation throughout the process which is conducive to potentially achieving high spatial accuracy. The \sysname utilizes a novel \ac{DSDF} block that performs dual scale feature exchange and a sub-network that exchanges multi-scale features using the \ac{DSDF} block. The \ac{DSDF} block takes two different scale inputs and employs a residual dense block that exchanges information across different scales after each convolutional layer in their corresponding dense blocks. The densely connected nature of blocks allows relevant high- and low-level features to be preserved for the final segmentation map prediction. 

% Suggestion: Combine these two paragraphs - same information repeating - try to sync and pass from one step to another - avoid repetition
%We also propose adding a complimentary gated shape stream that can leverage the combination of high- and low-level features to compute shape boundaries accurately. The multi-scale information exchange in our network preserves both high- and low-resolution feature representations, thereby producing finer, richer, and spatially accurate segmentation maps. The repeated multi-scale fusion helps in enhancing the high-resolution feature representations with the information propagated by low-resolution representations. Further, layers of residual networks allow redundant \ac{DSDF} blocks to die out, and only the most relevant extracted features contribute to the predicted segmentation maps. We have evaluated the \sysname segmentation model using four publicly available biomedical datasets. The results demonstrate that the proposed \sysname outperforms the {\color{red}\textsuperscript{$R_{3,2}$}\ac{SOTA}} segmentation methods on all standard computer vision evaluation metrics.}


% Connecting sentence is needed!!! Not clear why U-Net comes again! TODO!
% Either put with UNet or combine inside with connecting sentence
%ResUNet~\cite{zhang2018road} modified the U-Net architecture by adding residual connections to the standard convolutional units in the encoder and decoder, which eased the training of the network. This network was further studied in \cite{jha2019resunet++} where the authors modified ResUNet by adding ASPP, Squeeze and excitation units~\cite{hu2018squeeze} and attention mechanism to boost the performance of the network further.   
% When you write something: remember ask yourself context, importance, literature and novelty!!!
%


%A multi-scale contiguous memory mechanism is achieved by passing the input of a \ac{DSDF} block to every $\CLR$ operation of subsequent \ac{DSDF} blocks as in Figure~\ref{fig:smfrdbblock}.

% Note for a better contiguous memory mechanism you will need to have a memory management scheme!
% For example, you forget the past and and keep the present or use different memory storage e.g., encoding techniques such as latent space. But, you are not doing anything like that. Your gradients are flowing across all exchange layers, isn't it?
%

% \begin{algorithm}
% %\small
% \caption{ \ac{MSRF} sub-network} %\textbf{Algorithm 1:}
% \begin{algorithmic}[1]
% \STATE{Information exchange across all scales in \ac{MSRF} Sub-network}{}\\
% \STATE $N$ is no. of DSDF layers ($N=6$ in Fig.~\ref{fig:smfrdbblock}b) 
% \STATE  $H \gets {X_{\hat{h},1}, X_{\hat{h},3},X_{\hat{h}+1,1}, X_{\hat{h}+1,3},...}$ (High-res. input) \\
% \STATE  $L \gets {X_{\hat{l},2}, X_{\hat{l},4},X_{\hat{l}+1,2}, X_{\hat{l}+1,4},...}$ (Low-res. input)\\
% %\State $D$ (layer of MSRF sub-network). Set $D=2$
% %\State $\hat{h}\in\{1,2,3\}$ and $\hat{l}\in\{1,2,3\}$
% %\State $s:$ is resolution scale set $\{1,2,3,4\}$
% \STATE  $p\in\{1,3\}$ and $q\in\{2,4\}$ are scale pairs.
% %
% \FOR {$1\leq $N$ \leq 2$}
%     \STATE $X_{\hat{h}+1,p},X_{\hat{l}+1,q} = \DSDF(X_{\hat{h},p}, X_{\hat{l},q})$
% \ENDFOR
%     \STATE ${X}_{\hat{l}+2,2}, \tilde{X}_{\hat{h}+2,3} = \DSDF(X_{\hat{l}+1,2}, X_{\hat{h}+1,3} )$
%     \STATE $\tilde{X}_{\hat{l}, 2} = {X}_{\hat{l}+2,2}$, $\tilde{X}_{\hat{h}, 3} = {X}_{\hat{h}+2,3}$
% % \While {r \textless s-1}
% % \REPEAT 
% % \STATE{6 to 10 for layers 4 and 5}
% % Then use two DSDF blocks to output layers 4 and 5 h and l resolution features
% \WHILE {$4 \leq L \leq N-1$}
%     %\ForAll{$\mathit{\hat{h},\hat{l}} \in \mathit{H,L}$}
%     %\For $1\leq \text{DSDF} \leq 2$:
%     \STATE $X_{\hat{h}+1,p},X_{\hat{l}+1,q} = \DSDF(X_{\hat{h},p}, \tilde{X}_{\hat{l},q})$
%     %\STATE $X_{\hat{h}+1,p},X_{\hat{l}+1,q} = \DSDF(\tilde{X}_{\hat{h},3}, X_{\hat{l},q})$\\
    
%     \textbf{Update:}
%     \STATE $\tilde{X}_{\hat{l}, 2} = X_{\hat{l}+1,2}$, $\tilde{X}_{\hat{h}, 3}$ = $X_{\hat{h}+1,3}$
%     \STATE $X_{\hat{h},p} = X_{\hat{h}+1,p}$, $X_{\hat{l},q} = X_{\hat{l}+1,q}$
%     % \EndFor
 
 
%  %   \textbf{Exchange:} $\mathit{H1,L1} = \mathit{L,H}$
%     %
% %    \If{$\mathit{X_{\hat{h}+1,1}} \in \mathit{H}$}
% %        \State remove $\mathit{X_{\hat{h}+1,1}}~\text{from} ~\mathit{L{1}}$
% %        \State remove $\mathit{X_{\hat{l}+1,4}}~\text{from} ~\mathit{H{1}}$
% %    \EndIf
% %
% %    \If{$\mathit{X_{\hat{h}+1,1}} \notin \mathit{H}$}
% %        \State append $\mathit{X_{\hat{h}+1,1}}~\text{to}  ~\mathit{H{1}}$
% %        \State append $\mathit{X_{\hat{l}+1,4}}~\text{to} ~\mathit{L{1}}$
% %    \EndIf
%     %
% %\State \textbf{Exchange:} $\mathit{H,L} = \mathit{H1,L1}$
% \STATE {$L \gets L + 2$}
% \ENDWHILE
% \end{algorithmic}
% \label{alg:algo1}
% \end{algorithm}

% Required only main outcome, please move results to the result section
%We notice that using dice loss and binary cross-entropy loss individually decreases the performance of proposed \sysname. While training, using an equal weighted combination of \lbce and \ldcs in \lcomb gives a 1.58\% increase in mean \ac{DSC}, 2.37\% increase in mean \ac{mIoU}, 2.48\% decrease in mean recall, 5.23\% increase in mean precision as compared to the scenario where \lcomb = \lbce. Similarly, we obtain a increase of 3.56\% in mean \ac{DSC}, 4.68\% in mean \ac{mIoU}, 0.59\% in mean recall and 4.90\% in mean precision as opposed to the setting where \lcomb = \ldcs. It is evident that the combination of \ldcs and \lbce to supervise our network improves performance.} 


%we train the proposed \sysname using different scaling values of $w$ introduced in Equation~\ref{eq:5}.
% The aim is to understand the impact different scaling values have on the performance of \sysname. We can observe from Figure~\ref{fig:hyperparamw} that initially the \ac{DSC} is lower and drops the lowest when $w=0.3$. The highest \ac{DSC} is achieved when $w$ is set to $0.4$, and further increasing $w$ decreases \ac{DSC}.}
%
% {\color{red}\textsuperscript{$R_{2,3}$},\textsuperscript{$R_{4,5}$}Further, we have trained the proposed \sysname and a variant of \sysname to analyze the impact of the \ac{MSRF} sub-network on the shape stream. The variant model uses the shape stream before the \ac{MSRF} sub-network using only the features captured by the encoder. The \ac{MSRF} sub-network is placed after the shape-stream in the \sysname keeping the number of parameters same for both the models. The qualitative results (see Figure~\ref{fig:shapestream}) show that the \sysname can define precise and spatially accurate boundaries than the variant model. The variant model fails to recognize the boundaries of the target structure as it is deprived of the multi-scale features extracted by the \ac{MSRF} sub-network. This validates our choice of putting the MSRF sub-network before the shape stream block.



%Here, we can observe a significant improvement of 24.28\%, 33.75\%, 2.82\%, 6.30\% and 2.63\% in \ac{DSC} over ResUNet++, ResUNet++ + CRF, PraNet and the most recent methods (UACANet-S and UACANet-L), respectively. %}
% Network generalization results reported in Section~\ref{section:general} demonstrates the ability of our proposed \sysname to generalize better as compared to other \ac{SOTA} methods.

%which is only comparable to the performance of HRNetV2-W48 which gives a \ac{DSC} of 0.7901
% which is only comparable to the performance of HRNetV2-W48 which gives a \ac{DSC} of 0.7901


%\hl{usually segmenting most part of the region of interest with a high accuracy}, 
